Feedback Insertion-Deletion Codes

In this paper, a new problem of transmitting information over the adversarial insertion-deletion channel with feedback is introduced. Suppose that the encoder transmits $n$ binary symbols one-by-one over a channel, in which some symbols can be deleted and some additional symbols can be inserted. After each transmission, the encoder is notified about the insertions or deletions that have occurred within the previous transmission and the encoding strategy can be adapted accordingly. The goal is to design an encoder that is able to transmit error-free as much information as possible under the assumption that the total number of deletions and insertions is limited by $\tau n$, $0<\tau<1$. We show how this problem can be reduced to the problem of transmitting messages over the substitution channel. Thereby, the maximal asymptotic rate of feedback insertion-deletion codes is completely established. The maximal asymptotic rate for the adversarial substitution channel has been partially determined by Berlekamp and later finished by Zigangirov. However, the analysis of the lower bound by Zigangirov is quite complicated. We revisit Zigangirov's result and present a more elaborate version of his proof.

==> graphs.tex <==
% \begin{figure}[h!]
% \centering
%     \input{Graphs/timelinestyle}
%     \caption{Example for transition of the intervals $l(i), t(i)$, and $r(i)$ in case for a correct and incorrect transmission.}
%     \label{fig:interval-change-transistion}
% \end{figure}

% In Figure~\ref{fig:interval-change-transistion} one can see how the segments $l(i), r(i)$, and $t(i)$ change for the case of a correct and incorrect transmission. In particular, we see that the true segment is the one containing the point $\frac{1}{2}$. The segments left of $t(i)$ are summarized as $l(i)$ and on the right as $r(i)$. In the example a correct transmission is sending a "0", i.e. enlarging the intervals on the left of $\frac{1}{2}$ by $\beta$ and shrinking the right hand side by $\alpha$. We can see that there was a cross, since $l(i) < r(i)$ and now $l(i+1) > r(i+1)$. Moreover, since the transmission was correct we see that the true segment at step $i$ stays the true segment since it covers still the point $\frac{1}{2}$. In contrast, if the transmission was incorrect, i.e. enlarging by $\beta$ the right hand side of $\frac{1}{2}$ and shrinking the other part by $\alpha$, we observe that there was no cross and the true segment $t(i)$ does not contain the point $\frac{1}{2}$ anymore. Therefore, the true segment changes for time step $i+1$ and $T(i) \neq T(i+1)$.




% \begin{figure}
% \centering
% \begin{minipage}{.49\textwidth}
%   \centering
%     \input{Graphs/constants}
%      \caption{Illustration for different level sets for the function $u_1 (i)$ and $u_2(i)$ for $\tau = 0.15$, $\alpha = 2 \tau$, and $\beta = 2- \alpha$.}
%     \label{fig:levelsets-u1}
% \end{minipage}
% \hfill
% \begin{minipage}{.49\textwidth}
%   \centering
%     \input{Graphs/properties}
%   \caption{Illustration for the properties \emph{cross}, \emph{balanced}, and \emph{central} as functions of $l(i)$ and $r(i)$ when $\tau = 0.15, \alpha = 2 \tau$, and $\beta = 2- \alpha$.}
%     \label{fig:levelsets-props}
% \end{minipage}
% \end{figure}


% \begin{figure}
% \centering
% \begin{minipage}{.49\textwidth}
%   \centering
%     \input{Graphs/rainbow_u_funcs}
%      \caption{Illustration for level sets of the function $u(i)$ for $\tau = 0.15$, $\alpha = 2 \tau$, and $\beta = 2- \alpha$.}
%     \label{fig:levelsets-u-func-e}
% \end{minipage}
% \hfill
% \begin{minipage}{.49\textwidth}
%   \centering
%     \input{Graphs/rainbow_v_funcs}
%   \caption{Illustration for level sets of the function $v(i)$ for $\tau = 0.15$, $\alpha = 2 \tau$, and $\beta = 2- \alpha$.}
%     \label{fig:levelsets-v-func-e}
% \end{minipage}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \input{Graphs/trajectory}
%     \caption{Illustration for a trajectory of $t(i)$. We have $M = 2^{14}$ and transmit a random message, where we use $n^\prime = 27$ total transmissions. Errors occur at time steps 16, 21, and 22. Used parameters are $\tau = 0.15$, $\alpha = 2 \tau$, and $\beta = 2- \alpha$.}
%     \label{fig:trajectory}
% \end{figure}



% \begin{figure}[h!]
% \centering
%     \resizebox{.7\textwidth}{!}{
%     \input{Graphs/properties}
%     }
%     \caption{Illustration for the properties \emph{cross}, \emph{balanced}, and \emph{central} as functions of $l(i)$ and $r(i)$.}
%     \label{fig:levelsets-u1}
% \end{figure}

% \begin{figure}[h!]
% \centering
%     \resizebox{.7\textwidth}{!}{
%     \input{Graphs/levelsets}
%     }
%     \caption{Illustration for different level sets for the function $u_1 (i)$ for $\tau = 0.2$, $\alpha = 2 \tau$, and $\beta = 2- \alpha$.}
%     \label{fig:levelsets-u1}
% \end{figure}

% \begin{figure}[h!]
%     \centering
%     \resizebox{.7\textwidth}{!}{
%     \input{Graphs/uv_funcs}
%     }
%     \caption{Illustration for different level borders and example functions $u(i)$ and $v(i)$ for a time step $i$. Additionally, a trajectory for $t(i)$ for $n^\prime$ correct transmissions. Parameters are $\tau = 0.2$, $\alpha = 2 \tau$, and $\beta = 2- \alpha$.}
%     \label{fig:my_label}
% \end{figure}


%\resizebox{.7\textwidth}{!}{
%\input{Graphs/graph_t_u1_levels}
%}
